ORCA: A Challenging Benchmark for Arabic Language Understanding

Due to their crucial role in all NLP, several benchmarks have been proposed to evaluate pretrained language models. In spite of these efforts, no public benchmark of diverse nature currently exists for evaluation of Arabic. This makes it challenging to measure progress for both Arabic and multilingual language models. This challenge is compounded by the fact that any benchmark targeting Arabic needs to take into account the fact that Arabic is not a single language but rather a collection of languages and varieties. In this work, we introduce ORCA, a publicly available benchmark for Arabic language understanding evaluation. ORCA is carefully constructed to cover diverse Arabic varieties and a wide range of challenging Arabic understanding tasks exploiting 60 different datasets across seven NLU task clusters. To measure current progress in Arabic NLU, we use ORCA to offer a comprehensive comparison between 18 multilingual and Arabic language models. We also provide a public leaderboard with a unified single-number evaluation metric (ORCA score) to facilitate future research.

==> Comparison.tex <==
\subsection{Model Comparison}

We compare all the  multilingual language model (see Section~\ref{sec:Mult_LM}) and the Arabic pretrained language models (see Section~\ref{sec:Arabic_LM}) based on: (1) training data size,  (2) vocabulary size, (3)  language varieties, and (4) model configuration and architecture. Table~\ref{tab:models_config_comp}  shows a comparison between the models across these $4$ dimensions. 



==> deprecated-ORC_data_analysis.tex <==





\section{\ourbench~Data Distribution}\label{sec:SARLUE_analysis} 


\subsection{MSA vs. Dialect Distribution}

In order to analyze MSA-Dialect distribution in our \ourbench~benchmark,  we run an in-house  binary MSA-dialect classifier on all \ourbench~data splits (i.e., Train, Dev, and Test).\footnote{As our classifier is trained using \ourbench\textsubscript{DIA}, we exclude the \ourbench~dialect component from this analysis.}  For a deeper understanding of SuperARLUE data, we also calculate several measures including the average, median,  mode, and  type-token ratio (TTR) of the sentences in each task.  Table~\ref{tab:SuperARLUE_msa_dia}    shows the MSA Vs DIA data distribution and the statistical description of \ourbench~datasets.

\input{tables/SuperARLUE_MSA_Dia} 


\subsection{County-level Distribution}

We also acquire a country-level dialect distribution analysis using AraT5 model~\cite{nagoudi2021arat5} fine-tuned on the \ourbench~dialect country-level dataset (DIA-C). We run this country-level classifier only on the dialectal portion of \ourbench~(i.e., datasets that containing tweets predicted as dialect with MSA-dialect classifier). Figure~\ref{fig:map_countery} shows that  \ourbench~datasets are truly geographically diverse.\footnote{Again, the country-level classifier is also trained using \ourbench\textsubscript{DIA}, so we exclude the dialect tasks from this analysis.} 

%(see Appendix~\ref{appx:msa_vs_dia})

 

==> tables/Res_1.tex <==
\begin{table*}[t]
\centering

\begin{tabular}{lccccccc}
\toprule 
% \textbf{Dataset}     & \textbf{SOTA} & \textbf{mT5} & \textbf{AraT5\textsubscript{Tweet}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{AraT5\textsubscript{}} \\

\textbf{Dataset}     & \textbf{ARLUE\textsubscript{Senti}$^\star$ } & \textbf{ARLUE\textsubscript{SM}\textsuperscript{$\dagger$}} & \textbf{ARLUE\textsubscript{Topic}} & \textbf{ARLUE\textsubscript{Dia-B}} & \textbf{ARLUE\textsubscript{Dia-R}}  & \textbf{ARLUE\textsubscript{Dia-C}}  \\

% \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 

\toprule 
mBERT                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$    &	$92.79$ / $93.50$	                      \\
XLM-R &
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$    &	$92.79$ / $93.50$	                      \\ \hdashline 

GigaBERT &
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$    &	$92.79$ / $93.50$	                    \\ 

MARBRET                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$    &	$92.79$ / $93.50$	                                              \\


ARBERT &
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$    &	$92.79$ / $93.50$	                      \\
AraBERT                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$    &	$92.79$ / $93.50$                         \\
AraELEC. &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$
     &	$92.79$ / $93.50$	     \\ 
ArabicBERT                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$    &	$92.79$ / $93.50$	                      \\
Ar-ALBERT &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$
     &	$92.79$ / $93.50$	     \\ 
QARIB                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$    &	$92.79$ / $93.50$	                          \\
CAMeLBERT &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$
     &	$92.79$ / $93.50$	    \\ 
     

\toprule             
\end{tabular} \caption{Performance of our models on ARLUE TEST datasets (Acc / F$_1$). $^\star$ Metric for ARLUE\textsubscript{Senti} is Acc/ F\textsubscript{1}\textsuperscript{PN}. $^\ddagger$  Metric for ARLUE\textsubscript{QA} is Exact Match (EM) / F$_1$.$^\dagger$  ARLUE\textsubscript{SM}  results is the average score across the social meaning tasks. \textbf{SOTA:}  MARBERT~\cite{abdul2020arbert}. }


\label{tab:res1}
\end{table*}



==> tables/Res_2.tex <==
\begin{table*}[t]
\centering

\begin{tabular}{lccccccc}
\toprule 
% \textbf{Dataset}     & \textbf{SOTA} & \textbf{mT5} & \textbf{AraT5\textsubscript{Tweet}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{AraT5\textsubscript{}} \\

\textbf{Dataset}     & \textbf{ARLUE\textsubscript{QA}$^\ddagger$ } & \textbf{ARLUE\textsubscript{STS}\textsuperscript{$\dagger$}} & \textbf{ARLUE\textsubscript{NLI}} & \textbf{ARLUE\textsubscript{FC}} & \textbf{ARLUE\textsubscript{MGT}}   \\

% \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 

\toprule 
mBERT                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$         \\
XLM-R &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$
      \\ \hdashline 

GigaBERT &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$
   \\ 

MARBRET                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$                          \\


ARBERT &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$   \\ 
AraBERT                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$                          \\
AraELEC. &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$
         \\ 
ArabicBERT                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$                        \\
Ar-ALBERT &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$
       \\ 
QARIB                                          &   
$93.30$ / $94.00$	&	$92.46$ / $93.50$	&	$92.79$ / $93.50$	&	\bf$93.44$ / \bf$94.00$	&	$93.30$ / $94.00$                        \\
CAMeLBERT &
$81.60$ /$76.34$	&	$80.26$ / $73.59$	&	$80.41$ / $75.08$	&	\bf$ 81.97$ / \bf$ 76.60$	&	$81.09$ / $75.99$
      \\ 
     

\toprule             
\end{tabular} \caption{Performance of our models on ARLUE TEST datasets (Acc / F$_1$). $^\star$ Metric for ARLUE\textsubscript{Senti} is Acc/ F\textsubscript{1}\textsuperscript{PN}. $^\ddagger$  Metric for ARLUE\textsubscript{QA} is Exact Match (EM) / F$_1$.$^\dagger$  ARLUE\textsubscript{SM}  results is the average score across the social meaning tasks. \textbf{SOTA:}  MARBERT~\cite{abdul2020arbert}. }


\label{tab:res1}
\end{table*}



==> tables/Stat_Description_SARLUE.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\centering
 \renewcommand{\arraystretch}{0.9}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{llHcrrHrrr}
\hline
 \multirow{2}{*}{\textbf{Cluster}} &  \multirow{2}{*}{\textbf{Task}} & \multicolumn{4}{c}{\textbf{\#ARLUE}} & \multicolumn{4}{c}{\textbf{\#SuperARLUE}}                 \\ \cline {3-10}
 Cluster & Task  & \textbf{\#Datasets}&\textbf{#}   & \textbf{DEV} & \textbf{TEST}  & \textbf{\#Datasets} &\textbf{TRAIN}   & \textbf{DEV} & \textbf{TEST}                    \\ \hline 
 \multirow{7}{*}{\textbf{SC}}  &{Senti.} & $17$&  $190.9$K & $6.5$K  & $50$K & $\bf19$  & $50$K  & $5$K& $5$K   \\  
  &{SM~~} & $8$ &  $1.51$M  &  $162.5$K  & $166.1$K & $\bf9$  & $50$K  & $5$K & $5$K   \\  
 &Dia-B & $2$ &  $94.9$K & $10.8$K  & $12.9$K& $2$   & $50$K  & $5$K& $5$K   \\  
 &{Dia-R} & $2$ &  $38.5$K & $4.5$K  & $5.3$K& $\bf3$   & $38.5$K  & $4.5$K& $5$K   \\  
  &{Dia-C}  &$3$  &  $711.9$K & $31.5$K  & $52.1$K& $\bf4$   & $50$K  & $5$K& $5$K   \\ 
  & {CL} &  - &  - & -  & - & $\bf1$  & $3.2$K  & $0.9$K& $0.4$K   \\ 
  & {MG} &  - &  - & -  & - & $\bf1$ & $50$K  & $5$K& $5$K   \\   \hdashline  
\textbf{SP} & NER & $5$&  $277.7$K& $44.1$K & $66.5$K& $2$ & $5.2$K  & $1.1$K& $1.2$K   \\   \hdashline   
\textbf{TC} &Topic &$5$  &  $47.5$K & $5.9$K  & $5.9$K& $5$ & $47.5$K  & $5$K& $5$K   \\   \hdashline 

\hdashline 
\textbf{QA} & QA & $4$&  $101.6$K& $517$ & $7.4$K & $4$  & $50$K  & $5$K& $5$K   \\  \hline
\multirow{2}{*}{{\textbf{STSP}}} & {STS} & - &  - & -  & - & $\bf1$ & $0.8$K  & $0.2$K& $0.2$K   \\  
 &{XSTS} & - &  - & -  & - & $\bf1$ & $1.7$K  & $0.4$K& $0.2$K   \\ 
 &{QSTS} & - &  - & -  & - & $\bf1$ & $9.6$K  & $1.2$K& $1.2$K   \\ \hdashline 
\multirow{2}{*}{{\textbf{NLI}}}  &{XNLI}& - &  - & -  & - & $\bf1$  & $4.5$K  & $0.5$K& $2.5$K   \\  

 & {FC} &  - &  - & -  & - & $\bf2$  & $5$K  & $1$K& $1$K   \\ \toprule

\textbf{Total}  &  &  42 &  $2.9$M & $256$K  & $366$K  & $\bf57$ & $416$K  & $44.8$K& $46.7$K   \\ 
\toprule
% \multicolumn{6}{l}{}\\
% \multicolumn{6}{l}{}\\
\end{tabular}%
}
\caption{\small{A statistical description of the SuperARLUE data splits |Sent|  is the average sentences length by words, and TTR is type token-ratio.   }  }
\label{tab:SuperARLUE_msa_dia}
\end{table*}
%\multicolumn{4}{c}{\textbf{\#SuperARLUE}} 



==> tables/bAbI.tex <==
\begin{table}[h]

\resizebox{1\columnwidth}{!}{%
\centering
\begin{tabular}{lH} \toprule
\multicolumn{1}{c}{\textbf{Task}}            &\\ \toprule
Basic factoid QA with single supporting fact & WhereIsActor                            \\
Factoid QA with two supporting facts         & WhereIsObject                           \\
Factoid QA with three supporting facts       & WhereWasObject                          \\
Two argument relations: subject vs. object   & IsDir                                   \\
Three argument relations                     & WhoWhatGave                             \\
Yes/No questions                             & IsActorThere                            \\
Counting                                     & Counting                                \\
Lists/Sets                                   & Listing                                 \\
Simple Negation                              & Negation                                \\
Indefinite Knowledge                         & Indefinite                              \\
Basic coreference                            & BasicCoreference                        \\
Conjunction                                  & Conjunction                             \\
Compound coreference                         & CompoundCoreference                     \\
Time manipulation                            & Time                                    \\
Basic deduction                              & Deduction                               \\
Basic induction                              & Induction                               \\
Positional reasoning                         & PositionalReasoning                     \\
Reasoning about size                         & Size                                    \\
Path finding                                 & PathFinding                             \\
Reasoning about agent's motivation           & Motivations                             \\ \toprule
\end{tabular}}\caption{The bAbI tasks as described in their original paper~\cite{weston2015towards}}\label{tab:bAbI}
\end{table}

==> tmp_biblio.tex <==
@inproceedings{levesque2012winograd,
  title={The winograd schema challenge},
  author={Levesque, Hector and Davis, Ernest and Morgenstern, Leora},
  booktitle={Thirteenth International Conference on the Principles of Knowledge Representation and Reasoning},
  year={2012}
}


@inproceedings{haim2006second,
  title={The second pascal recognising textual entailment challenge},
  author={Haim, R Bar and Dagan, Ido and Dolan, Bill and Ferro, Lisa and Giampiccolo, Danilo and Magnini, Bernardo and Szpektor, Idan},
  booktitle={Proceedings of the Second PASCAL Challenges Workshop on Recognising Textual Entailment},
  year={2006}
}


@article{wang2019superglue,
  title={Superglue: A stickier benchmark for general-purpose language understanding systems},
  author={Wang, Alex and Pruksachatkun, Yada and Nangia, Nikita and Singh, Amanpreet and Michael, Julian and Hill, Felix and Levy, Omer and Bowman, Samuel R},
  journal={arXiv preprint arXiv:1905.00537},
  year={2019},
  url={https://papers.nips.cc/paper/2019/hash/4496bf24afe7fab6f046bf4923da8de6-Abstract.html}
}


@inproceedings{lan2020gigabert,
  author     = {Lan, Wuwei and Chen, Yang and Xu, Wei and Ritter, Alan},
  title      = {GigaBERT: Zero-shot Transfer Learning from English to Arabic},
  booktitle  = {Proceedings of The 2020 Conference on Empirical Methods on Natural Language Processing (EMNLP)},
  year       = {2020}
} 

      
@inproceedings{mohammad2018semeval,
  title={Semeval-2018 task 1: Affect in tweets},
  author={Mohammad, Saif and Bravo-Marquez, Felipe and Salameh, Mohammad and Kiritchenko, Svetlana},
  booktitle={Proceedings of the 12th international workshop on semantic evaluation},
  pages={1--17},
  year={2018}
}

@inproceedings{Mohammad2018semeval,
  title={{Semeval-2018 Task 1: Affect in Tweets}},
  author={Mohammad, S. Bravo-Marquez and F. Salameh, M. and Kiritchenko, S.},
  booktitle={Proceedings of International Workshop on Semantic Evaluation (SemEval-2018)},
  year={2018},
  organization={Association for Computational Linguistics},
  url={https://www.aclweb.org/anthology/S18-1001.pdf}
}


@InProceedings{DARWISH12018
  author = {Kareem Darwish ,Hamdy Mubarak ,Ahmed Abdelali ,Mohamed Eldesouki ,Younes Samih ,Randah Alharbi ,Mohammed Attia ,Walid Magdy and Laura Kallmeyer},
  title = {Multi-Dialect Arabic POS Tagging: A CRF Approach},
  booktitle = {Proceedings of the Eleventh International Conference on Language Resources and Evaluation (LREC 2018)},
  year = {2018},
  month = {may},
  date = {7-12},
  location = {Miyazaki, Japan},
  editor = {Nicoletta Calzolari (Conference chair) and Khalid Choukri and Christopher Cieri and Thierry Declerck and Sara Goggi and Koiti Hasida and Hitoshi Isahara and Bente Maegaard and Joseph Mariani and Hélène Mazo and Asuncion Moreno and Jan Odijk and Stelios Piperidis and Takenobu Tokunaga},
  publisher = {European Language Resources Association (ELRA)},
  address = {Paris, France},
  isbn = {979-10-95546-00-9},
  language = {english}
  }
  
@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher and others},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}

@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}

@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher and others},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}

@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}

@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher and others},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}


@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}

@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher and others},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}

@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}

@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher and others},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}
@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean Y and Chuang, Jason and Manning, Christopher D and Ng, Andrew Y and Potts, Christopher},
  booktitle={Proceedings of the conference on empirical methods in natural language processing (EMNLP)},
  volume={1631},
  pages={1642},
  year={2013},
  organization={Citeseer}
}
@inproceedings{wang2018glue,
  title={Glue: A multi-task benchmark and analysis platform for natural language understanding},
  author={Wang, Alex and Singh, Amanpreet and Michael, Julian and Hill, Felix and Levy, Omer and Bowman, Samuel R},
   booktitle = "Proceedings of the 2018 {EMNLP} Workshop {B}lackbox{NLP}: Analyzing and Interpreting Neural Networks for {NLP}",
    month = nov,
    year = "2018",
    address = "Brussels, Belgium",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/W18-5446",
    doi = "10.18653/v1/W18-5446",
    pages = "353--355"
}

















































